A Fast Deep Learning Model for Textual Relevance in Biomedical Information Retrieval

Publications in the life sciences are characterized by a large technical vocabulary, with many lexical and semantic variations for expressing the same concept. Towards addressing the problem of relevance in biomedical literature search, we introduce a deep learning model for the relevance of a document's text to a keyword style query. Limited by a relatively small amount of training data, the model uses pre-trained word embeddings. With these, the model first computes a variable-length Delta matrix between the query and document, representing a difference between the two texts, which is then passed through a deep convolution stage followed by a deep feed-forward network to compute a relevance score. This results in a fast model suitable for use in an online search engine. The model is robust and outperforms comparable state-of-the-art deep learning approaches.

==> full_tables.tex <==
%%%
%%% Full tables saved here
%%%

\begin{table}
\small
\begin{center}
\begin{tabular}{$l^l^l^l^l^l}
\toprule
{} & NDCG.20 & MAP & Prec.5 & Prec.10 & Prec.20 \\
\midrule
rev DocID	          & 0.141	& 0.455	& 0.344	& 0.375	& 0.406	\\
BM25-Title$^1$	 & 0.325	& 0.567	& 0.591	& 0.549	& 0.502 \\
UQLM-Title	        & 0.314	& 0.560	& 0.574	& 0.541	& 0.500 \\
WMD-Title$^2$	& 0.329$^{=1}$	& 0.579$^{+1}$	& 0.603$^{+1}$	& 0.564	& 0.516 \\
\midrule
DRMM	               & 0.300$^{-1}$	& 0.545$^{-1}$	& 0.549$^{-1}$	& 0.526	& 0.492 \\
SevMos-C1$^3$	& 0.352$^{+2}$	& 0.597$^{+2}$	& 0.625$^{+2}$	& 0.587	& 0.537 \\
SevMos-C3$^4$	& 0.373$^{+3}$	& 0.594$^{=3,+2}$	& 0.626$^{=3,+2}$	& 0.585	& 0.531 \\
\midrule
Delta-32$^5$	   & 0.365$^{+3,-4}$	& 0.601$^{+3,4}$	& 0.634$^{+3,4}$	& 0.593	& 0.540 \\
Delta-32-Lex3	\rowstyle{\bfseries}  & 0.394$^{+4,5}$	& 0.609$^{+4,5}$	& 0.646$^{+4,5}$	& 0.600	& 0.541 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:Metrics.Full}Ranking metrics on the Full Test Data. \textmd{The superscripts indicate statistical comparisons: `+' for increase, '-' for decrease, '=' for equivalent, to a 99\% confidence using a paired t-test. The comparison baselines are indicated with numbers 1 through 5, as marked in the first column. Highest values are in bold.}}
\end{table}

\begin{table}
\small
\begin{center}
\begin{tabular}{$l^l^l^l^l^l}
\toprule
{} & NDCG.20 & MAP & Prec.5 & Prec.10 & Prec.20 \\
\midrule
rev DocID           & 0.081 & 0.413 & 0.310 & 0.335 & 0.365 \\
BM25-Title$^1$ & 0.233 & 0.474 & 0.490 & 0.461 & 0.431 \\
WMD-Title$^2$  & 0.243$^{+1}$ & 0.483$^{+1}$ & 0.496$^{=1}$ & 0.470 & 0.440 \\
\midrule
DRMM                 & 0.242$^{+1,=2}$ & 0.461$^{-1,2}$ & 0.462$^{-1,2}$ & 0.450 & 0.427 \\
SevMos-C1$^3$  & 0.290$^{+2}$ & 0.510$^{+2}$ & 0.538$^{+2}$ & 0.508 & 0.469 \\
SevMos-C3$^4$  & 0.304$^{+2,3}$ & 0.502$^{+2,-3}$ & 0.535$^{+2,=3}$ & 0.504 & 0.464 \\
\midrule
Delta-32$^5$     & 0.296$^{+2,=3}$ & 0.513$^{+2,=3}$ & 0.550$^{+2,3}$ & 0.515 & 0.476 \\
Delta-32-Lex3 \rowstyle{\bfseries}    & 0.326$^{+4,5}$ & 0.522$^{+4,5}$ & 0.560$^{+4,5}$ & 0.523 & 0.479 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:Metrics.Neg20plus}Ranking metrics on the `Neg20+' Test Data}
\end{table}


\begin{table}
\small
\begin{center}
\begin{tabular}{$l^l^l^l^l^l}
\toprule
{} & NDCG.20 & MAP & Prec.5 & Prec.10 & Prec.20 \\
\midrule
rev DocID & 0.191 & 0.488 & 0.364 & 0.407 & 0.442 \\
BM25-Title$^1$ & 0.333 & 0.593 & 0.604 & 0.565 & 0.521 \\
WMD-Title$^2$ & 0.330$^{=1}$ & 0.603$^{+1}$ & 0.614$^{+1}$ & 0.583 & 0.534 \\
\midrule
DRMM & 0.318$^{-1}$ & 0.580$^{-1}$ & 0.578$^{-1}$ & 0.551 & 0.521 \\
SevMos-C1$^3$ & 0.358$^{+2}$ & 0.624$^{+2}$ & 0.642$^{+2}$ & 0.606 & 0.558 \\
SevMos-C3$^4$ & 0.375$^{+2,3}$ & 0.621$^{+2,=3}$ & 0.640$^{+2,=3}$ & 0.602 & 0.549 \\
\midrule
Delta-32$^5$ & 0.382$^{+3}$ & 0.629$^{=3}$ & 0.648$^{=3}$ & 0.608 & 0.559 \\
Delta-32-Lex3 \rowstyle{\bfseries}  & 0.413$^{+4,5}$ & 0.638$^{+4,5}$ & 0.666$^{+4,5}$ & 0.619 & 0.560 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:Metrics.OneNewWord}Ranking metrics on the `OneNewWord' Test Data. \textmd{The significance for DRMM's NDCG.20 comparison is to a confidence of 95\%.}}
\end{table}


\begin{table}
\small
\begin{center}
\begin{tabular}{$l^l^l^l^l^l}
\toprule
{} & NDCG.20 & MAP & Prec.5 & Prec.10 & Prec.20 \\
\midrule
rev DocID           & 0.195 & 0.508 & 0.389 & 0.438 & 0.466 \\
BM25-Title$^1$ & 0.309 & 0.581 & 0.586 & 0.561 & 0.521 \\
WMD-Title$^2$  & 0.306$^{=1}$ & 0.590$^{+1}$ & 0.595$^{=1}$ & 0.577 & 0.536 \\
\midrule
DRMM                 & 0.311$^{=1,2}$ & 0.578$^{=1,-2}$ & 0.570$^{=1,-2}$ & 0.553 & 0.526 \\
SevMos-C1$^3$ & 0.344$^{+2}$ & 0.615$^{+2}$ & 0.624$^{+2}$ & 0.598 & 0.557 \\
SevMos-C3$^4$ & 0.355$^{+2,=3}$ & 0.614$^{+2,=3}$ & 0.632$^{+2,=3}$ & 0.597 & 0.550 \\
\midrule
Delta-32$^5$     & 0.362$^{+3,=4}$ & 0.622$^{+3,4}$ & 0.638$^{=3,4}$ & 0.609 & 0.564 \\
Delta-32-Lex3 \rowstyle{\bfseries}  & 0.400$^{+4,5}$ & 0.633$^{+4,5}$ & 0.661$^{+4,5}$ & 0.622 & 0.566 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:Metrics.OneNewWord}Ranking metrics on the `AllNewWords' Test Data}
\end{table}

